Optional P\'olya trees: posterior rates and uncertainty quantification

We consider statistical inference in the density estimation model using a tree-based Bayesian approach, with Optional P\'olya trees as prior distribution. We derive near-optimal convergence rates for corresponding posterior distributions with respect to the supremum norm. For broad classes of H\"older-smooth densities, we show that the method automatically adapts to the unknown H\"older regularity parameter. We consider the question of uncertainty quantification by providing mathematical guarantees for credible sets from the obtained posterior distributions, leading to near-optimal uncertainty quantification for the density function, as well as related functionals such as the cumulative distribution function. The results are illustrated through a brief simulation study.

==> Arxiv OPT/opt_inference_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{amsmath,amssymb}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Commands/macros IC

\usepackage{color, latexsym}


\usepackage{esint}
\usepackage{dsfont}

\usepackage{nccmath}



\newcommand{\ra}{\rightarrow}{}
\def\1{1\!{\rm l}}

\newcommand{\leqa}{\lesssim}
\newcommand{\geqa}{\gtrsim}

\newcommand{\EM}{\ensuremath}
\newcommand{\bP}{\EM{\mathbf{P}}}
\newcommand{\bE}{\EM{\mathbf{E}}}
\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\ze}{\zeta}
\newcommand{\ep}{\epsilon}
\newcommand{\ga}{\gamma}
\newcommand{\Ga}{\Gamma}
\newcommand{\g}{\gamma}
\newcommand{\la}{\lambda}
\newcommand{\La}{\Lambda}
\newcommand{\om}{\omega}
\newcommand{\ph}{\Phi}
\newcommand{\si}{\sigma}
\newcommand{\te}{\theta}
\newcommand{\ta}{\tau}
\newcommand{\veps}{\varepsilon}
\newcommand{\vphi}{\varphi}
\newcommand{\pli}{+\infty}

\newcommand{\cA}{\EM{\mathcal{A}}}
\newcommand{\cB}{\EM{\mathcal{B}}}
\newcommand{\cC}{\EM{\mathcal{C}}}
\newcommand{\cD}{\EM{\mathcal{D}}}
\newcommand{\cE}{\EM{\mathcal{E}}}
\newcommand{\cF}{\EM{\mathcal{F}}}
\newcommand{\cG}{\EM{\mathcal{G}}}
\newcommand{\cH}{\EM{\mathcal{H}}}
\newcommand{\cI}{\EM{\mathcal{I}}}
\newcommand{\cJ}{\EM{\mathcal{J}}}
\newcommand{\cK}{\EM{\mathcal{K}}}
\newcommand{\cL}{\EM{\mathcal{L}}}
\newcommand{\cM}{\EM{\mathcal{M}}}
\newcommand{\cN}{\EM{\mathcal{N}}}
\newcommand{\cP}{\EM{\mathcal{P}}}
\newcommand{\cQ}{\EM{\mathcal{Q}}}
\newcommand{\cR}{\EM{\mathcal{R}}}
\newcommand{\cS}{\EM{\mathcal{S}}}
\newcommand{\cT}{\EM{\mathcal{T}}}
\newcommand{\cU}{\EM{\mathcal{U}}}
\newcommand{\cV}{\EM{\mathcal{V}}}
\newcommand{\cW}{\EM{\mathcal{W}}}
\newcommand{\cX}{\EM{\mathcal{X}}}
\newcommand{\cY}{\EM{\mathcal{Y}}}
\newcommand{\cZ}{\EM{\mathcal{Z}}}
 
\newcommand{\psg}{{\langle}}
\newcommand{\psd}{{\rangle}}
\newcommand{\varf}[1]{\mathbf{Var}_{#1}}

\newcommand{\bl}[1]{\textcolor[rgb]{0.00,0.00,1.00}{#1}}
\newcommand{\ve}[1]{\textcolor[rgb]{0.00,1.00,0.00}{#1}}
\newcommand{\gris}[1]{\textcolor[RGB]{136,152,206}{#1}}
\newcommand{\ora}[1]{\textcolor[rgb]{1.00,0.50,0.00}{#1}}

\definecolor{blendedblue}{rgb}{0.2,0.2,0.7}
\newcommand{\sbl}[1]{{\color{blendedblue}{#1}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\newcommand{\rap}{\overset{{\bf P}}{\rightarrow}}
\newcommand{\noi}{\noindent}
\newcommand{\bk}{\backslash}

\newcommand{\bp}{\mathbb{P}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\zed}{\mathbb{Z}}
\newcommand{\mb}{\mathbb{B}}
\newcommand{\mh}{\mathbb{H}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\tri}{\triangleq}
\newcommand{\N}{\mathbb{N}}

\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lac}{\left\{}
\newcommand{\rac}{\right\}}

\newcommand{\given}{\,|\,}

\newcommand{\ble}[1]{{\color{blue}{#1}}}
\newcommand{\re}[1]{{\color{red}{#1}}}
\newcommand{\gr}[1]{{\color{green}{#1}}}
\newcommand{\pur}[1]{{\color{purple}{#1}}}
\newcommand{\gra}[1]{{\color{gray}{#1}}}
\newcommand{\ma}[1]{{\color{magenta}{#1}}}


\newcommand{\erp}{\mathbb{R}^{+}}
\newcommand{\bfi}{\bar{\Phi}} 

\newcommand{\vep}{\varepsilon_n}

\newcommand{\R}{\mathds{R}}
\newcommand{\ind}{\mathds{1}}

\newcommand{\paa}{\lfloor \alpha \rfloor} 

\newcommand{\rn}{\sqrt{n}}
\newcommand{\nm}{n^{-1/2}}

\newcommand{\cl}{\rightsquigarrow} 

\newcommand{\vp}{\vspace{.5cm}}

\newcommand{\hal}{\hat\al}
\newcommand{\hatha}{\hat\theta_\al}

\newcommand{\bet}{\operatorname{Beta}}
\newcommand{\bel}{\operatorname{Be}}
\newcommand{\kl}{\operatorname{KL}}

\newcommand{\bi}{\begin{enumerate}[label=\roman*)]}
\newcommand{\ei}{\end{enumerate}}
\newcommand{\ba}{\begin{array}{rcl}}
\newcommand{\ea}{\end{array}}
\newcommand{\di}{\displaystyle}

\def\bT{\mathbb{T}}
\def\mT{\mathcal{T}}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


% Macros/commandes Thibault
\usepackage{tikz}
\newcommand\RBox[1]{%
  \tikz\node[draw,rounded corners,align=center,] {#1};%
}

\usetikzlibrary{arrows,positioning, calc}
\tikzstyle{vertex}=[draw,fill=black!15,circle,minimum size=20pt,inner sep=0pt]


\usepackage{mathtools}
\usepackage{caption}
\usepackage{subcaption}


% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{example}{Example}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newsiamthm{prop}{Proposition}

% Sets running headers as well as PDF title and authors
\headers{Optional PTs: rates and UQ}{I. Castillo and T. Randrianarisoa}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Optional P\'olya trees: posterior rates and uncertainty quantification\thanks{Submitted to the editors October 2021.
\funding{This work was funded by the ANR, project ANR-17-CE40-0001 (BASICS).}}}

% Authors: full names plus addresses.
\author{Isma\"el Castillo\thanks{LPSM Sorbonne \& IUF 
  (\email{ismael.castillo@upmc.fr}, \url{https://www.lpsm.paris/pageperso/castillo//}).}
\and Thibault Randrianarisoa \thanks{LPSM Sorbonne 
  (\email{thibault.randrianarisoa@sorbonne-universite.fr}, \url{https://thibaultrandrianarisoa.netlify.app}).}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}




%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

